Real-Time Dispatching of Large-Scale Ride-Sharing Systems: Integrating Optimization, Machine Learning, and Model Predictive Control

This paper considers the dispatching of large-scale real-time ride-sharing systems to address congestion issues faced by many cities. The goal is to serve all customers (service guarantees) with a small number of vehicles while minimizing waiting times under constraints on ride duration. This paper proposes an end-to-end approach that tightly integrates a state-of-the-art dispatching algorithm, a machine-learning model to predict zone-to-zone demand over time, and a model predictive control optimization to relocate idle vehicles. Experiments using historic taxi trips in New York City indicate that this integration decreases average waiting times by about 30% over all test cases and reaches close to 55% on the largest instances for high-demand zones.

==> mpc-framework.tex <==
\section{A MPC Framework for Real-Time Dial-A-Ride with Relocation} \label{sec:mpc-framework}
The model predictive control framework's goal is to relocate vehicles to zones of future predicted demand.
A zone is a geographic region which allows the optimization to make aggregate decisions for relocating vehicles.
The framework has three components: the first is a demand forecasting model;
the second component, vehicle allocation, uses the predicted demand in a mixed-integer program which determines the number of vehicles to move from one zone to another;
the last component, vehicle relocation, is a mixed-integer program which, for each zone, determines which specific idle vehicles to move to every other zone, based on the number of vehicles obtained in component two.
This procedure is run every $\omega \geq 1$ epochs.
While a vehicle is relocating, it cannot be assigned to any requests, therefore,
$\omega$ must be picked to strike a balance between relocating idle vehicles often enough to preempt demand, but infrequently enough to allow idle vehicles to be assigned to new requests.


